A pair of Jones polynomial positivity obstructions

We provide a new bound on the maximum degree of the Jones polynomial of a positive link with second Jones coefficient equal to $\pm 1$ or $\pm 2$. This builds upon the result of our previous work, in which we found such a bound for positive fibered links. We also show that each of these three bounds obstruct positivity for infinitely many almost-positive diagrams, allowing us to classify infinitely many knots as almost-positive.

==> bib.tex <==
\begin{thebibliography}{999}

\bibitem[AT17]{AT17}
Tetsuya Abe and Keiji Tagami, \textit{Characterization of positive links and the $s$-invariant for links}, Canadian Journal of Mathematics, 69(6), 1201-1218. doi:10.4153/CJM-2016-030-7 (2017). arXiv:1405.4061 [math.GT]

\bibitem[Ad+92]{Ad+}
Colin C. Adams, Jeffrey F. Brock, John Bugbee, Timothy D. Comar, Keith A. Faigin, Amy M. Huston, Anne M. Joseph and David Pesikoff, \textit{Almost alternating links}, Topology and its Applications 46 (1992).
%, available at \url{https://core.ac.uk/download/pdf/82039133.pdf}.


\bibitem[DES09]{Di+}
 Yuanan Diao, Claus Ernst, and Andrzej Stasiak, \textit{A Partial Ordering of Knots Through Diagrammatic Unknotting},
Journal of Knot Theory and Its Ramifications Vol. 18, No. 04, pp. 505-522 (2009).
% 2006, available at \url{https://math.charlotte.edu/sites/math.charlotte.edu/files/fields/preprint_archive/paper/2006_12_0.pdf}.

\bibitem[Fut13]{Fut13} 
David Futer, \textit{Fiber detection for state surfaces,} Algebr. Geom. Topol. 13 (2013), no. 5,
2799–2807. 	arXiv:1201.1643 [math.GT]


\bibitem[FKP13]{FKP13} 
David Futer, Efstratia Kalfagianni, and Jessica Purcell, \textit{Guts of surfaces and the colored
Jones polynomial,} Lecture Notes in Mathematics, vol. 2069, Springer, Heidelberg, 2013. arXiv:1108.3370 [math.GT]

 
\bibitem[Kau87]{Kauffman} 
Louis H. Kauffman, \textit{State Models and the Jones Polynomial}, Topology: Vol. 26 No. 3 (1987), 395-407.

\bibitem[KI]{KnotInfo}
C. Livingston and A. H. Moore, KnotInfo: Table of Knot Invariants, knotinfo.math.indiana.edu, April 7, 2022.


\bibitem[St]{Stoimenow}
A. Stoimenow, \textit{On Polynomials and Surfaces of Variously Positive Links}, 	Jour. Europ. Math. Soc. 7(4) (2005), 477--509. arXiv:math/0202226 [math.GT]

\bibitem[St05]{St05}
A. Stoimenow, \textit{On Some Restrictions to the Values of the Jones Polynomial}, Indiana University Mathematics Journal , 2005, Vol. 54, No. 2 (2005), pp. 557-574.

\bibitem[St22]{St22}
A. Stoimenow, \textit{Applications of Jones semiadequacy tests}, 2022.\\
{http://stoimenov.net/stoimeno/homepage/papers.html}

\bibitem[StW]{StW}
A. Stoimenow, Lists of non-alternating positive of crossing number $\leq 15$ ,\\ {http://stoimenov.net/stoimeno/homepage/ptab/index.html}

\bibitem[Th87]{Thistlethwaite}
Morwen B. Thistlethwaite,  \textit{A Spanning Tree Expansion of the Jones Polynomial}, Topology: Vol. 26 No. 3 (1987).
%, available at \url{https://www.maths.ed.ac.uk/~v1ranick/papers/thistlewaitejones.pdf}.


\end{thebibliography}
